MILE: A Multi-Level Framework for Scalable Graph Embedding

Recently there has been a surge of interest in designing graph embedding methods. Few, if any, can scale to a large-sized graph with millions of nodes due to both computational complexity and memory requirements. In this paper, we relax this limitation by introducing the MultI-Level Embedding (MILE) framework -- a generic methodology allowing contemporary graph embedding methods to scale to large graphs. MILE repeatedly coarsens the graph into smaller ones using a hybrid matching technique to maintain the backbone structure of the graph. It then applies existing embedding methods on the coarsest graph and refines the embeddings to the original graph through a graph convolution neural network that it learns. The proposed MILE framework is agnostic to the underlying graph embedding techniques and can be applied to many existing graph embedding methods without modifying them. We employ our framework on several popular graph embedding techniques and conduct embedding for real-world graphs. Experimental results on five large-scale datasets demonstrate that MILE significantly boosts the speed (order of magnitude) of graph embedding while generating embeddings of better quality, for the task of node classification. MILE can comfortably scale to a graph with 9 million nodes and 40 million edges, on which existing methods run out of memory or take too long to compute on a modern workstation. Our code and data are publicly available with detailed instructions for adding new base embedding methods: \url{https://github.com/jiongqian/MILE}.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table1.tex <==
\begin{table}[!htb]
%For Dataset PPI
\subfloat[PPI Dataset\label{tab1:PPI}]{
  \resizebox{0.5\columnwidth}{!}{
\begin{tabular}{l|l|l|l}
\hline \hline
\textbf{Method} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Time (mins)} \\
\hline
DeepWalk  & 23.0  & 18.6  & 2.42   \\
MILE (DeepWalk, $m=1$)  & 25.6\footnotesize{(11.3\%$\uparrow$)} & 20.4\footnotesize{(9.7\%$\uparrow$)}  & 1.22\footnotesize{(2.0$\times$)}   \\
MILE (DeepWalk, $m=2$)  & 25.5\footnotesize{(10.9\%$\uparrow$)} & 20.7\footnotesize{(11.3\%$\uparrow$)} & 0.67\footnotesize{(3.6$\times$)}   \\
% Harp (DeepWalk, $m=1$)    &   24.1 \footnotesize{(4.8\%$\uparrow$)}   &   20.2 \footnotesize{(8.6\%$\uparrow$)}   &   3.08 \footnotesize{(0.8$\times$)}  \\
% Harp (DeepWalk, $m=2$)    &   24.2 \footnotesize{(5.2\%$\uparrow$)}   &   20.4 \footnotesize{(9.7\%$\uparrow$)}   &   4.00 \footnotesize{(0.6$\times$)}  \\
\hline
Node2Vec  & 24.3  & 19.6  & 4.01   \\
MILE (Node2Vec, $m=1$)  & 25.9\footnotesize{(6.6\%$\uparrow$)}  & 20.6\footnotesize{(5.1\%$\uparrow$)}  & 1.77\footnotesize{(2.3$\times$)}   \\
MILE (Node2Vec, $m=2$)  & 26.0\footnotesize{(7.0\%$\uparrow$)}  & {\it 21.1}\footnotesize{(7.7\%$\uparrow$)}  & 0.98\footnotesize{(4.1$\times$)}   \\
\hline
Line    &   25.0    &   19.5     &   2.27  \\
MILE (Line, $m=1$)    &   25.8 \footnotesize{(3.2\%$\uparrow$)}    &   19.8 \footnotesize{(1.5\%$\uparrow$)}    &   1.22 \footnotesize{(1.9$\times$)}  \\
MILE (Line, $m=2$)    &   24.7 \footnotesize{(-1.2\%$\downarrow$)}    &   19.0 \footnotesize{(-2.6\%$\downarrow$)}    &   0.68 \footnotesize{(3.3$\times$)}  \\
% Harp (Node2Vec, $m=1$)    &   22.3 \footnotesize{(-8.2\%$\downarrow$)}    &   18.4 \footnotesize{(-6.1\%$\downarrow$)}    &   3.90 \footnotesize{(1.0$\times$)}  \\
% Harp (Node2Vec, $m=2$)    &   22.2 \footnotesize{(-8.6\%$\downarrow$)}    &   18.8 \footnotesize{(-4.1\%$\downarrow$)}    &   4.68 \footnotesize{(0.9$\times$)}  \\
\hline
GraRep  & 25.5  & 20.0  & 2.99   \\
MILE (GraRep, $m=1$)  & 25.6\footnotesize{(0.4\%$\uparrow$)}  & 19.8\footnotesize{(-1.0\%$\downarrow$)} & 1.11\footnotesize{(2.7$\times$)}   \\
MILE (GraRep, $m=2$)  & 25.3\footnotesize{(-0.8\%$\downarrow$)} & 19.5\footnotesize{(-2.5\%$\downarrow$)} & 0.43\footnotesize{(6.9$\times$)}   \\
\hline
NetMF & 24.6  & 20.1  & 0.65   \\
MILE (NetMF, $m=1$)  & {\bf 26.9}\footnotesize{(9.3\%$\uparrow$)}  & {\bf 21.6}\footnotesize{(7.5\%$\uparrow$)}  & 0.27\footnotesize{(2.5$\times$)}   \\
MILE (NetMF, $m=2$)  & {\it 26.7}\footnotesize{(8.5\%$\uparrow$)}  & {\it 21.1}\footnotesize{(5.0\%$\uparrow$)}  & 0.17\footnotesize{(3.9$\times$)}   \\
\hline \hline 
\end{tabular}}
}
%For Dataset Blog
\subfloat[Blog Dataset\label{tab1:Blog}]{
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{l|l|l|l}
\hline \hline
\textbf{Method} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Time (mins)} \\
\hline
DeepWalk  & 37.0  & 21.0  & 8.02   \\
MILE (DeepWalk, $m=1$)  & {\it 42.9}\footnotesize{(15.9\%$\uparrow$)} & {\it 27.0}\footnotesize{(28.6\%$\uparrow$)} & 4.69\footnotesize{(1.7$\times$)}   \\
MILE (DeepWalk, $m=2$)  & 39.4\footnotesize{(6.5\%$\uparrow$)}  & 23.5\footnotesize{(11.9\%$\uparrow$)} & 2.71\footnotesize{(3.0$\times$)}   \\
% Harp (DeepWalk, $m=1$)    &   41.3 \footnotesize{(11.6\%$\uparrow$)}  &   27.2 \footnotesize{(29.5\%$\uparrow$)}  &   9.85 \footnotesize{(0.8$\times$)}  \\
% Harp (DeepWalk, $m=2$)    &   42.0 \footnotesize{(13.5\%$\uparrow$)}  &   27.8 \footnotesize{(32.4\%$\uparrow$)}  &   14.70 \footnotesize{(0.5$\times$)}  \\
\hline
Node2Vec  & 39.1  & 23.0  & 13.04  \\
MILE (Node2Vec, $m=1$)  & 42.8\footnotesize{(9.5\%$\uparrow$)}  & 26.4\footnotesize{(14.8\%$\uparrow$)} & 6.99\footnotesize{(1.9$\times$)}   \\
MILE (Node2Vec, $m=2$)  & 40.2\footnotesize{(2.8\%$\uparrow$)}  & 23.9\footnotesize{(3.9\%$\uparrow$)}  & 3.89\footnotesize{(3.4$\times$)}   \\
\hline
Line    &   39.1    &   22.6     &   5.95  \\
MILE (Line, $m=1$)    &   38.4 \footnotesize{(-1.8\%$\downarrow$)}    &   21.0 \footnotesize{(-7.0\%$\downarrow$)}    &   3.84 \footnotesize{(1.55$\times$)}  \\
MILE (Line, $m=2$)    &   37.3 \footnotesize{(-4.6\%$\downarrow$)}    &   19.6 \footnotesize{(-13.2\%$\downarrow$)}    &   2.58 \footnotesize{(2.31$\times$)}  \\
% Harp (Node2Vec, $m=1$)    &   36.2 \footnotesize{(-7.4\%$\downarrow$)}    &   22.1 \footnotesize{(-3.9\%$\downarrow$)}    &   13.16 \footnotesize{(1.0$\times$)}  \\
% Harp (Node2Vec, $m=2$)    &   37.3 \footnotesize{(-4.6\%$\downarrow$)}    &   23.0 \footnotesize{(0.0\%$\uparrow$)}   &   17.26 \footnotesize{(0.8$\times$)}  \\
\hline
GraRep  & 40.6  & 23.3  & 28.76  \\
MILE (GraRep, $m=1$)  & 41.7\footnotesize{(2.7\%$\uparrow$)}  & 24.0\footnotesize{(3.0\%$\uparrow$)}  & 12.25\footnotesize{(2.3$\times$)}  \\
MILE (GraRep, $m=2$)  & 38.3\footnotesize{(-5.7\%$\downarrow$)} & 20.4\footnotesize{(-12.4\%$\downarrow$)}  & 4.22\footnotesize{(6.8$\times$)}   \\
\hline
NetMF & 41.4  & 25.0  & 2.64   \\
MILE (NetMF, $m=1$)  & {\bf 43.8}\footnotesize{(5.8\%$\uparrow$)}  & {\bf 27.6}\footnotesize{(10.4\%$\uparrow$)} & 1.98\footnotesize{(1.3$\times$)}   \\
MILE (NetMF, $m=2$)  & 42.4\footnotesize{(2.4\%$\uparrow$)}  & 25.5\footnotesize{(2.0\%$\uparrow$)}  & 1.27\footnotesize{(2.1$\times$)}   \\
\hline \hline 
\end{tabular}}
} \\ 

%For Dataset flickr
\subfloat[Flickr Dataset\label{tab1:Flickr}]{
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{l|l|l|l}
\hline \hline
\textbf{Method} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Time (mins)} \\
\hline
DeepWalk  & 40.0  & 26.5  & 50.08  \\
MILE (DeepWalk, $m=1$)  & {\it 40.4}\footnotesize{(1.0\%$\uparrow$)}  & {\it 27.3}\footnotesize{(3.0\%$\uparrow$)}  & 34.48\footnotesize{(1.5$\times$)}  \\
MILE (DeepWalk, $m=2$)  & 39.3\footnotesize{(-1.8\%$\downarrow$)} & 26.1\footnotesize{(-1.5\%$\downarrow$)} & 26.88\footnotesize{(1.9$\times$)}  \\
% Harp (DeepWalk, $m=1$)    &   40.6 \footnotesize{(1.5\%$\uparrow$)}   &   28.7 \footnotesize{(8.3\%$\uparrow$)}   &   83.60 \footnotesize{(0.6$\times$)}  \\
% Harp (DeepWalk, $m=2$)    &   40.7 \footnotesize{(1.7\%$\uparrow$)}   &   28.6 \footnotesize{(7.9\%$\uparrow$)}   &   105.40 \footnotesize{(0.5$\times$)}  \\
\hline
Node2Vec  & 40.5  & 27.3  & 78.21  \\
MILE (Node2Vec, $m=1$)  & {\bf 40.7}\footnotesize{(0.5\%$\uparrow$)}  & {\bf 27.7}\footnotesize{(1.5\%$\uparrow$)}  & 50.54\footnotesize{(1.5$\times$)}  \\
MILE (Node2Vec, $m=2$)  & 38.8\footnotesize{(-4.2\%$\downarrow$)} & 25.8\footnotesize{(-5.5\%$\downarrow$)} & 36.85\footnotesize{(2.1$\times$)}  \\
\hline
Line    &   34.0    &   14.5     &   60.42  \\
MILE (Line, $m=1$)    &   33.9 \footnotesize{(-0.3\%$\downarrow$)}    &   13.8 \footnotesize{(-4.8\%$\downarrow$)}    &   30.24 \footnotesize{(2.00$\times$)}  \\
MILE (Line, $m=2$)    &   33.3 \footnotesize{(-2.1\%$\downarrow$)}    &   12.9 \footnotesize{(-11.0\%$\downarrow$)}    &   19.05 \footnotesize{(3.17$\times$)}  \\
% Harp (Node2Vec, $m=1$)    &   40.5 \footnotesize{(0.0\%$\uparrow$)}   &   28.5 \footnotesize{(4.4\%$\uparrow$)}   &   101.12 \footnotesize{(0.8$\times$)}  \\
% Harp (Node2Vec, $m=2$)    &   40.4 \footnotesize{(-0.2\%$\downarrow$)}    &   28.4 \footnotesize{(4.0\%$\uparrow$)}   &   122.43 \footnotesize{(0.6$\times$)}  \\
\hline
GraRep  & N/A & N/A & $>$ 2343.37  \\
MILE (GraRep, $m=1$)  & 36.7  & 18.6  & 697.39\footnotesize{($>$3.4$\times$)}  \\
MILE (GraRep, $m=2$)  & 36.3  & 18.6  & 163.05\footnotesize{($>$14.4$\times$)}   \\
\hline
NetMF\footnotemark  & 31.8  & 14.0  & 69.72  \\
MILE (NetMF, $m=1$)  & 39.3\footnotesize{(23.6\%$\uparrow$)} & 24.5\footnotesize{(75.0\%$\uparrow$)} & 24.03\footnotesize{(2.9$\times$)}  \\
MILE (NetMF, $m=2$)  & 39.5\footnotesize{(24.2\%$\uparrow$)} & 25.9\footnotesize{(85.0\%$\uparrow$)} & 15.84\footnotesize{(4.4$\times$)}  \\
\hline \hline 
\end{tabular}}
}
%For Dataset youtube
\subfloat[YouTube Dataset\label{tab1:YouTube}]{
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{l|l|l|l}
\hline \hline
\textbf{Method} & \textbf{Micro-F1} & \textbf{Macro-F1} & \textbf{Time (mins)} \\
\hline
DeepWalk  & 45.2  & 34.7  & 604.83   \\
MILE (DeepWalk, $m=6$)  & 46.1\footnotesize{(2.0\%$\uparrow$)}  & {\bf 38.5}\footnotesize{(11.0\%$\uparrow$)} & 55.20\footnotesize{(11.0$\times$)}   \\
MILE (DeepWalk, $m=8$)  & 44.3\footnotesize{(-2.0\%$\downarrow$)} & 35.3\footnotesize{(1.7\%$\uparrow$)}  & 37.35\footnotesize{(16.2$\times$)}   \\
% Harp (DeepWalk, $m=6$)    &   46.6 \footnotesize{(3.1\%$\uparrow$)}   &   {\bf 38.6}\footnotesize{(11.2\%$\uparrow$)}  &   1727.78 \footnotesize{(0.4$\times$)}  \\
% Harp (DeepWalk, $m=8$)    &   N/A &   N/A &   N/A  \\
\hline
Node2Vec  & 45.5  & 34.6  & 951.27   \\
MILE (Node2Vec, $m=6$)  & {\bf 46.3}\footnotesize{(1.8\%$\uparrow$)}  & {\it 38.3}\footnotesize{(10.7\%$\uparrow$)} & 83.52\footnotesize{(11.4$\times$)}   \\
MILE (Node2Vec, $m=8$)  & 44.3\footnotesize{(-2.6\%$\downarrow$)} & 35.8\footnotesize{(3.5\%$\uparrow$)}  & 55.55\footnotesize{(17.1$\times$)}   \\
\hline
Line    &   46.0    &   35.0     &   583.37  \\
MILE (Line, $m=6$)    &   {\it 46.2} \footnotesize{(0.4\%$\uparrow$)}    &   36.2 \footnotesize{(3.4\%$\uparrow$)}    &   53.97 \footnotesize{(10.81$\times$)}  \\
MILE (Line, $m=8$)    &   44.4 \footnotesize{(-3.5\%$\downarrow$)}    &   35.7 \footnotesize{(2.0\%$\uparrow$)}    &   33.41 \footnotesize{(17.46$\times$)}  \\
% Harp (Node2Vec, $m=6$)    &   47.2 \footnotesize{(3.7\%$\uparrow$)}   &   38.9 \footnotesize{(12.4\%$\uparrow$)}  &   1981.33 \footnotesize{(0.5$\times$)}  \\
% Harp (Node2Vec, $m=8$)    &   N/A &   N/A &   N/A  \\
\hline
GraRep  & N/A & N/A & $>$ 3167.00  \\ % the number is based on level=5.
MILE (GraRep, $m=6$)  & 43.2  & 32.7  & 1644.89\footnotesize{($>$1.9$\times$)}   \\
MILE (GraRep, $m=8$)  & 42.3  & 30.9  & 673.95\footnotesize{($>$4.7$\times$)}  \\
\hline
NetMF & N/A & N/A & $>$ 574.75   \\ % the number is estimated on the time error happening. yo-raw_NE.pbs.o2520482
MILE (NetMF, $m=6$)  & 40.9  & 27.8  & 35.22\footnotesize{($>$16.3$\times$)}  \\
MILE (NetMF, $m=8$)  & 39.2  & 25.5  & 19.22\footnotesize{($>$29.9$\times$)}  \\
\hline \hline 
\end{tabular}}
} \\ 
%\vspace{-2mm}
\caption{
%\small{
Performance of MILE. %compared to the original embedding methods. 
DeepWalk, Node2Vec, GraRep, and NetMF denotes the original method without using our MILE framework. $m$ is  the number of coarsening levels.
%  to $1$ and $2$ for PPI, Blog and Flickr, while choosing $6$ and $8$ for YouTube (due to its larger scale). 
%The Micro-F1 and Macro-F1 are in \underline{$10^{-2}$} scale while the column Time shows the running time in minutes. 
The numbers within the parenthesis by the reported Micro-F1 and Macro-F1 scores are the \textit{\underline{relative percentage}} of change compared to the original method
%, e.g., MILE (DeepWalk, $m=1$) vs. DeepWalk. ``$\uparrow$'' and ``$\downarrow$'' respectively indicate improvement and decline. 
Numbers along with ``$\times$'' is the speedup compared to the original method. ``N/A'' indicates the method runs out of memory and we show the amount of running time spent when it happens.%}
}
\label{tab1}
% \vspace{1em}
\end{table}


==> table1short.tex <==
\begin{table}
%For Dataset PPI
\subfloat[PPI Dataset\label{tab1:PPI}]{
  \resizebox{0.5\columnwidth}{!}{
\begin{tabular}{l|l|l}
\hline \hline
\textbf{Method} & \textbf{Micro-F1} & \textbf{Time (mins)} \\
\hline
DeepWalk  & 23.0    & 2.4   \\
MILE (DeepWalk, $m=1$)  & 25.6 \footnotesize{(11.3\%$\uparrow$)}  & 1.2 \footnotesize{(2.0$\times$)}   \\
MILE (DeepWalk, $m=2$)  & 25.5 \footnotesize{(10.9\%$\uparrow$)}  & 0.6 \footnotesize{(3.6$\times$)}   \\
% Harp (DeepWalk, $m=1$)    &   24.1 \footnotesize{(4.8\%$\uparrow$)}   &   20.2 \footnotesize{(8.6\%$\uparrow$)}   &   3.08 \footnotesize{(0.8$\times$)}  \\
% Harp (DeepWalk, $m=2$)    &   24.2 \footnotesize{(5.2\%$\uparrow$)}   &   20.4 \footnotesize{(9.7\%$\uparrow$)}   &   4.00 \footnotesize{(0.6$\times$)}  \\
\hline
Node2Vec  & 24.3   & 4.01   \\
MILE (Node2Vec, $m=1$)  & 25.9 \footnotesize{(6.6\%$\uparrow$)}   & 1.7 \footnotesize{(2.3$\times$)}   \\
MILE (Node2Vec, $m=2$)  & 26.0 \footnotesize{(7.0\%$\uparrow$)}    & 0.9 \footnotesize{(4.1$\times$)}   \\
\hline
Line    &   25.0    &   2.2  \\
MILE (Line, $m=1$)    &   25.8 \footnotesize{(3.2\%$\uparrow$)}       &   1.2 \footnotesize{(1.9$\times$)}  \\
MILE (Line, $m=2$)    &   24.7 \footnotesize{(-1.2\%$\downarrow$)}      &   0.6 \footnotesize{(3.3$\times$)}  \\
% Harp (Node2Vec, $m=1$)    &   22.3 \footnotesize{(-8.2\%$\downarrow$)}    &   18.4 \footnotesize{(-6.1\%$\downarrow$)}    &   3.90 \footnotesize{(1.0$\times$)}  \\
% Harp (Node2Vec, $m=2$)    &   22.2 \footnotesize{(-8.6\%$\downarrow$)}    &   18.8 \footnotesize{(-4.1\%$\downarrow$)}    &   4.68 \footnotesize{(0.9$\times$)}  \\
\hline
GraRep  & 25.5   & 2.9   \\
MILE (GraRep, $m=1$)  & 25.6 \footnotesize{(0.4\%$\uparrow$)}   & 1.1 \footnotesize{(2.7$\times$)}   \\
MILE (GraRep, $m=2$)  & 25.3 \footnotesize{(-0.8\%$\downarrow$)} & 0.43 \footnotesize{(6.9$\times$)}   \\
\hline
NetMF & 24.6   & 0.6   \\
MILE (NetMF, $m=1$)  & {\bf 26.9} \footnotesize{(9.3\%$\uparrow$)}    & 0.2 \footnotesize{(2.5$\times$)}   \\
MILE (NetMF, $m=2$)  & {26.7} \footnotesize{(8.5\%$\uparrow$)}  & 0.1 \footnotesize{(3.9$\times$)}   \\
\hline \hline 
\end{tabular}}
}
%For Dataset Blog
\subfloat[Blog Dataset\label{tab1:Blog}]{
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{l|l|l}
\hline \hline
\textbf{Method} & \textbf{Micro-F1} & \textbf{Time (mins)} \\
\hline
DeepWalk  & 37.0  & 8.0   \\
MILE (DeepWalk, $m=1$)  &  42.9 \footnotesize{(15.9\%$\uparrow$)} & 4.6 \footnotesize{(1.7$\times$)}   \\
MILE (DeepWalk, $m=2$)  & 39.4 \footnotesize{(6.5\%$\uparrow$)}   & 2.7 \footnotesize{(3.0$\times$)}   \\
% Harp (DeepWalk, $m=1$)    &   41.3 \footnotesize{(11.6\%$\uparrow$)}  &   27.2 \footnotesize{(29.5\%$\uparrow$)}  &   9.85 \footnotesize{(0.8$\times$)}  \\
% Harp (DeepWalk, $m=2$)    &   42.0 \footnotesize{(13.5\%$\uparrow$)}  &   27.8 \footnotesize{(32.4\%$\uparrow$)}  &   14.70 \footnotesize{(0.5$\times$)}  \\
\hline
Node2Vec  & 39.1   & 13.0  \\
MILE (Node2Vec, $m=1$)  & 42.8 \footnotesize{(9.5\%$\uparrow$)}   & 6.9 \footnotesize{(1.9$\times$)}   \\
MILE (Node2Vec, $m=2$)  & 40.2 \footnotesize{(2.8\%$\uparrow$)}    & 3.8 \footnotesize{(3.4$\times$)}   \\
\hline
Line    &   39.1    &   5.9  \\
MILE (Line, $m=1$)    &   38.4 \footnotesize{(-1.8\%$\downarrow$)}        &   3.8  \footnotesize{(1.55$\times$)}  \\
MILE (Line, $m=2$)    &   37.3 \footnotesize{(-4.6\%$\downarrow$)}        &   2.5  \footnotesize{(2.31$\times$)}  \\
% Harp (Node2Vec, $m=1$)    &   36.2 \footnotesize{(-7.4\%$\downarrow$)}    &   22.1 \footnotesize{(-3.9\%$\downarrow$)}    &   13.16 \footnotesize{(1.0$\times$)}  \\
% Harp (Node2Vec, $m=2$)    &   37.3 \footnotesize{(-4.6\%$\downarrow$)}    &   23.0 \footnotesize{(0.0\%$\uparrow$)}   &   17.26 \footnotesize{(0.8$\times$)}  \\
\hline
GraRep  & 40.6  & 28.7   \\
MILE (GraRep, $m=1$)  & 41.7 \footnotesize{(2.7\%$\uparrow$)}  & 12.2 \footnotesize{(2.3$\times$)}  \\
MILE (GraRep, $m=2$)  & 38.3 \footnotesize{(-5.7\%$\downarrow$)} & 4.2 \footnotesize{(6.8$\times$)}   \\
\hline
NetMF & 41.4  & 2.6   \\
MILE (NetMF, $m=1$)  & {\bf 43.8} \footnotesize{(5.8\%$\uparrow$)}   & 1.9 \footnotesize{(1.3$\times$)}   \\
MILE (NetMF, $m=2$)  & 42.4 \footnotesize{(2.4\%$\uparrow$)}   & 1.2 \footnotesize{(2.1$\times$)}   \\
\hline \hline 
\end{tabular}}
} \\ 

%For Dataset flickr
\subfloat[Flickr Dataset\label{tab1:Flickr}]{
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{l|l|l}
\hline \hline
\textbf{Method} & \textbf{Micro-F1}  & \textbf{Time (mins)} \\
\hline
DeepWalk  & 40.0  & 50.0  \\
MILE (DeepWalk, $m=1$)  & {40.4} \footnotesize{(1.0\%$\uparrow$)}   & 34.4 \footnotesize{(1.5$\times$)}  \\
MILE (DeepWalk, $m=2$)  & 39.3 \footnotesize{(-1.8\%$\downarrow$)}  & 26.8 \footnotesize{(1.9$\times$)}  \\
% Harp (DeepWalk, $m=1$)    &   40.6 \footnotesize{(1.5\%$\uparrow$)}   &   28.7 \footnotesize{(8.3\%$\uparrow$)}   &   83.60 \footnotesize{(0.6$\times$)}  \\
% Harp (DeepWalk, $m=2$)    &   40.7 \footnotesize{(1.7\%$\uparrow$)}   &   28.6 \footnotesize{(7.9\%$\uparrow$)}   &   105.40 \footnotesize{(0.5$\times$)}  \\
\hline
Node2Vec  & 40.5  & 78.2   \\
MILE (Node2Vec, $m=1$)  & {\bf 40.7} \footnotesize{(0.5\%$\uparrow$)}    & 50.5 \footnotesize{(1.5$\times$)}  \\
MILE (Node2Vec, $m=2$)  & 38.8 \footnotesize{(-4.2\%$\downarrow$)}  & 36.8 \footnotesize{(2.1$\times$)}  \\
\hline
Line    &   34.0    &   60.4   \\
MILE (Line, $m=1$)    &   33.9  \footnotesize{(-0.3\%$\downarrow$)}    &   30.2  \footnotesize{(2.00$\times$)}  \\
MILE (Line, $m=2$)    &   33.3 \footnotesize{(-2.1\%$\downarrow$)}     &   19.0  \footnotesize{(3.17$\times$)}  \\
% Harp (Node2Vec, $m=1$)    &   40.5 \footnotesize{(0.0\%$\uparrow$)}   &   28.5 \footnotesize{(4.4\%$\uparrow$)}   &   101.12 \footnotesize{(0.8$\times$)}  \\
% Harp (Node2Vec, $m=2$)    &   40.4 \footnotesize{(-0.2\%$\downarrow$)}    &   28.4 \footnotesize{(4.0\%$\uparrow$)}   &   122.43 \footnotesize{(0.6$\times$)}  \\
\hline
GraRep  & N/A & $>$ 2343.3   \\
MILE (GraRep, $m=1$)  & 36.7  & 697.3  \footnotesize{($>$3.4$\times$)}  \\
MILE (GraRep, $m=2$)  & 36.3  & 163.0  \footnotesize{($>$14.4$\times$)}   \\
\hline
NetMF  & 31.8   & 69.7   \\
MILE (NetMF, $m=1$)  & 39.3 \footnotesize{(23.6\%$\uparrow$)}  & 24.0 \footnotesize{(2.9$\times$)}  \\
MILE (NetMF, $m=2$)  & 39.5 \footnotesize{(24.2\%$\uparrow$)}  & 15.8 \footnotesize{(4.4$\times$)}  \\
\hline \hline 
\end{tabular}}
}
%For Dataset youtube
\subfloat[YouTube Dataset\label{tab1:YouTube}]{
\resizebox{0.5\columnwidth}{!}{
\begin{tabular}{l|l|l}
\hline \hline
\textbf{Method} & \textbf{Micro-F1} & \textbf{Time (mins)} \\
\hline
DeepWalk  & 45.2  & 604.8    \\
MILE (DeepWalk, $m=6$)  & 46.1 \footnotesize{(2.0\%$\uparrow$)}  & 55.2 \footnotesize{(11.0$\times$)}   \\
MILE (DeepWalk, $m=8$)  & 44.3 \footnotesize{(-2.0\%$\downarrow$)} & 37.3 \footnotesize{(16.2$\times$)}   \\
% Harp (DeepWalk, $m=6$)    &   46.6 \footnotesize{(3.1\%$\uparrow$)}   &   {\bf 38.6}\footnotesize{(11.2\%$\uparrow$)}  &   1727.78 \footnotesize{(0.4$\times$)}  \\
% Harp (DeepWalk, $m=8$)    &   N/A &   N/A &   N/A  \\
\hline
Node2Vec  & 45.5  & 951.2    \\
MILE (Node2Vec, $m=6$)  & {\bf 46.3} \footnotesize{(1.8\%$\uparrow$)}  & 83.5 \footnotesize{(11.4$\times$)}   \\
MILE (Node2Vec, $m=8$)  & 44.3 \footnotesize{(-2.6\%$\downarrow$)} & 55.5 \footnotesize{(17.1$\times$)}   \\
\hline
Line    &   46.0    &   583.3   \\
MILE (Line, $m=6$)    &   {46.2} \footnotesize{(0.4\%$\uparrow$)}   &   53.9  \footnotesize{(10.81$\times$)}  \\
MILE (Line, $m=8$)    &   44.4 \footnotesize{(-3.5\%$\downarrow$)}     &   33.4  \footnotesize{(17.46$\times$)}  \\
% Harp (Node2Vec, $m=6$)    &   47.2 \footnotesize{(3.7\%$\uparrow$)}   &   38.9 \footnotesize{(12.4\%$\uparrow$)}  &   1981.33 \footnotesize{(0.5$\times$)}  \\
% Harp (Node2Vec, $m=8$)    &   N/A &   N/A &   N/A  \\
\hline
GraRep  & N/A & $>$ 3167.0  \\ % the number is based on level=5.
MILE (GraRep, $m=6$)  & 43.2  & 1644.8  \footnotesize{($>$1.9$\times$)}   \\
MILE (GraRep, $m=8$)  & 42.3  & 673.9 \footnotesize{($>$4.7$\times$)}  \\
\hline
NetMF & N/A & $>$ 574.7   \\ % the number is estimated on the time error happening. yo-raw_NE.pbs.o2520482
MILE (NetMF, $m=6$)  & 40.9  & 35.2 \footnotesize{($>$16.3$\times$)}  \\
MILE (NetMF, $m=8$)  & 39.2  & 19.2 \footnotesize{($>$29.9$\times$)}  \\
\hline \hline 
\end{tabular}}
} \\ 
%\vspace{-2mm}
\caption{
%\small{
Performance of MILE. %compared to the original embedding methods. 
DeepWalk, Node2Vec, GraRep, and NetMF denotes the original method without using our MILE framework. $m$ is  the number of coarsening levels.
%  to $1$ and $2$ for PPI, Blog and Flickr, while choosing $6$ and $8$ for YouTube (due to its larger scale). 
%The Micro-F1 and Macro-F1 are in \underline{$10^{-2}$} scale while the column Time shows the running time in minutes. 
The numbers within the parenthesis by the reported Micro-F1 scores are the \textit{\underline{relative percentage}} of change compared to the original method
%, e.g., MILE (DeepWalk, $m=1$) vs. DeepWalk. ``$\uparrow$'' and ``$\downarrow$'' respectively indicate improvement and decline. 
Numbers along with ``$\times$'' is the speedup compared to the original method. ``N/A'' indicates the method runs out of memory and we show the amount of running time spent when it happens.%}
}
\label{tab1}
\end{table}

